OrcoDCS: An IoT-Edge Orchestrated Online Deep Compressed Sensing Framework

Compressed data aggregation (CDA) over wireless sensor networks (WSNs) is task-specific and subject to environmental changes. However, the existing compressed data aggregation (CDA) frameworks (e.g., compressed sensing-based data aggregation, deep learning(DL)-based data aggregation) do not possess the flexibility and adaptivity required to handle distinct sensing tasks and environmental changes. Additionally, they do not consider the performance of follow-up IoT data-driven deep learning (DL)-based applications. To address these shortcomings, we propose OrcoDCS, an IoT-Edge orchestrated online deep compressed sensing framework that offers high flexibility and adaptability to distinct IoT device groups and their sensing tasks, as well as high performance for follow-up applications. The novelty of our work is the design and deployment of IoT-Edge orchestrated online training framework over WSNs by leveraging an specially-designed asymmetric autoencoder, which can largely reduce the encoding overhead and improve the reconstruction performance and robustness. We show analytically and empirically that OrcoDCS outperforms the state-of-the-art DCDA on training time, significantly improves flexibility and adaptability when distinct reconstruction tasks are given, and achieves higher performance for follow-up applications.

==> Back_Introduction.tex <==
\section{Introduction}
\label{sec: introduction}

% disadvantages of traditional method: collect all data and compute in the cloud
% 1. data is not easy to collect
% 2. privacy issue
% 3. require considerable communication and storage cost. in addition, centralized computing requires powerful computing server
%

% FL advantage
% 1. similar to crowdsourcing, data is collected by the user devices
% 2. keep data privacy
% 3. in-network computing, reducing the transmission cost
%

% challenge
% 1. trade-off between data quality, computing expenditure, and data transfer time
%    select the suitable # users to jointly satisfy the data size requirement and minimize computing expenditure (MKP)
%    meanwhile, user data may be biased --> a larger emd usually indicates a lower accuracy of trained model
%    the more data, the better accuracy, but may lead to the higher expenditure
%    a user with higher-quality data may take a much longer time for transmission
% 2. parameter upload scheduling with multiple antennas (makespan minimization with identical machines) -> obscure training cost
%    not only scheduling, but also selection
% 3. 


{\color{red}
Nowadays, the ever-expanding demands for Artificial Intelligence (AI) have drawn more and more focus around the world. 
A great number of distinct applications \cite{GoogleVoice,AlexNet,Mario,DeepLink,PredictingLearnerInteractions,Experience-DrivenNetworking} are becoming a critical part of human being's daily life. 
However, due to the data-intensive property of current AI models, the general models would need to consume individually personal data to turn its generalized representations into specific ones(e.g. Google uses machine learning model to improve word candidates accuracy on personal mobile devices\cite{KeyboardQuery}), thereby raising several data-related concerns. 
First, the security of data. Since data stored typically in personal computers and mobile devices may associate sensitive personal information, habits and locations, the owners of data might feel reluctant to share with third parties.
%no obvious correlations one another).
For example, in order to improve user experience many websites would ask for permission for obtaining clients history data when they are browsing its sites.
Second, on the basis of the first issue, specific data cannot be shared out of personal devices. In other words, in order to take advantage of these data, corresponding computations should be performed within local devices with limited computation capabilities. Compared with cloud computing systems, local devices would take much time completing computations. Relevant outcomes that contain none of personal data would be sent back to the servers belonging to third parties, thereby posing another issue. 
Lastly, due to the indispensable communications between local devices and servers, transmission efficiency that poses impact on completion time should be carefully taken into account. Now that the data on mobile devices represent more personal information compared with personal computers. Therefore, in this paper, wireless communications are mainly expected. 



%Catastrophic Forgetting
%an apparent tendency of research 
To alleviate the above issues, Federated Learning sheds light on decentralized data training framework \cite{FederatedLearning}.
%mathematical
%which provides multiple outputs for an input in one run to simultaneously solve multiple tasks.
In this brand-new training framework, Server(s) send global model(s) to local devices(i.e. through wireless connections) and the devices train the model(s) with its local data set. After finishing training, the devices send back the outcomes to the server(s) where the outcomes only serve as an update improving global models'  parameters stored in the server(s) and no personal information is included. Compared with centralized training framework, several conclusions can be acquired: 1) Data and computations are distributed among numerous devices taking part in training global models. Each device might be responsible for little training. That is, servers are no longer to be memory-intensive and computing-intensive. 2) Data security can be guaranteed since the data considered are always stored in local memories instead of being sent to data centers for training. 3) With more personal data considered, third parties may make it better to offer personal services and recommendations with respect to each client where it is a win-win situation.


Although Federated Learning framework fulfills the hope of decentralized training some difficulties have been discovered. For example, devices' communication and computation capabilities influence overall training time since Federated Learning requests servers to update its global model(s) parameters as soon as receiving all the updates from devices. That is to say, the device with the worse capabilities would prolong the training process. \cite{ClientSelection} offers a client selection algorithm based on heterogeneous resources in mobile edge. Apart from mobile edge resources issue, transmission time is another factor worthy considering. From servers' perspective, if global model(s) can be downsized or transformed before sending to mobile devices, transmission overhead can be lower. From mobile devices' perspective, if the structure of update can be simplified or sparsified before sending back to servers transmission overhead can be much lower. \cite{ExpandningtheReach} and \cite{ImprovingCommunicationEfficiency} illustrate respectively server-to-client and client-to-server approaches to diminish the size of data to be transmitted. \cite{OverTheAir} makes use of signal processing methods to improve transmissions between servers and clients(i.e. mobile devices). Two concerns above are mainly training-time-related. Nevertheless, the most critical issue of Federated Learning framework is the downgrade of accuracy resulting from \emph{Non-IID data} on each device. \cite{Non-IID} shows that if data distributions on the clients selected are extremely polarized(i.e. a majority of clients contain only one or two classes of data) testing accuracy would be rather disappointing. All the research above has offered brilliant approaches with respect to specific issues. Nonetheless, the interplay between heterogeneous resources in mobile edges, data distributions and transmission has not been clearly inspected before. For instance, \cite{AgnosticFL} proposes an new Federated-Learning-like framework with data distributions on clients considered while transmission issues have not been detailed. \cite{OverTheAir} exploits the property of wireless multiple-access channel to accelerate the aggregation of local updates while specific data distributions are not considered. In particular, relevant costs of executing Federated Learning are a practical problem worthy researching and optimizing. That is to say, an one-size-fits-all optimization algorithm leveraging transmissions, data distributions, number of clients selected and costs has not been explored in the literature, thereby giving the motivation for this paper.



Simultaneously optimizing transmissions time, data distribution, amount of data(i.e. number of clients) and relevant costs for updating the global model(s) stored in the server(s) arises several new research challenges as follows.

% data數量
1) \emph{\challengeCPTradeOff}. \cite{CooperativeSGD,FederatedLearning} show that the more clients are involved in training the better the convergence rate and prediction accuracy. In this paper, the number of clients selected are regarded as the amount of data selected. Since more data come with more costs(e.g. more money to be spent) it is impractical to obtain better parameters without considering corresponding costs. 
% scheduling, computation and transmissions
2) \emph{\challengeHeteroresources}. \cite{ClientSelection,Non-IID} claim that the heterogeneous resources(i.e. transmission capabilities and data quality) in edge devices would make great impact on overall training efficiency and accuracy. More specifically, Consider the limited number of antennas equipped by servers, devices transmission scheduling problem arises. Moreover, data quality(i.e. data distribution)\footnote{The metric for data distribution is called EMD(Earth mover's distance).} is proved to be the main factor biasing the parameters for global models. 
% EMD, empirical distribution and data distribution of clients 的距離
3) \emph{\challengeIndetrainingcost}. Consider a set of devices, jointly computing  training expenditure and overall transmission time to obtain total training cost in polynomial time is nature. Nevertheless, it is NP-hard to acquire to compute the minimum transmission time over multiple antennas.  That is, the problem becomes quite challenging since device selection should take into account overall transmission time. 

To address the above challenges, we present a new optimization problem, termed \ProblemName\ (\ProblemNameAbbr).
With the following given parameters including: 1) each devices' computation and transmission capabilities, 2) first-round update from each client and 3) quantity of data from each client. \ProblemNameAbbr\ simultaneously determines a set of clients to share global model(s) for training and pre-schedules the transmission sequence over the finite bandwidth to minimize the total cost that consists of: 1) transmission, 2) data quantity for training and 3) incentive for clients with quality data distribution, while ensuring \emph{data quantity requirement} (i.e., data quantity should exceed user requirement) and \emph{performance requirement constraint} (i.e., the distance between empirical and data distribution should satisfy user reqiurement).

We prove that \ProblemNameAbbr\ is NP-hard.
% 這些 hardness results 還需要確認，大概先寫個樣子
For \ProblemNameAbbr, we design a $3$-approximation algorithm, called \AlgoName\ (\AlgoNameAbbr), to obtain the asymptotically optimal bound.
To achieve \emph{\challengeHeteroresources}, \AlgoNameAbbr\
sets the different restrictions to device transmission time to generate different candidate solutions for avoiding selecting devices with overlength transmission time. In addition, \AlgoNameAbbr\ sets up a threshold. If a device with EMD lower than that, it would not be a candidate. By doing so, efficiency and quality can be guaranteed. 
% among them.
Moreover, for each candidate solution, \AlgoNameAbbr\ incorporates Primal-Dual technique into selecting appropriate devices that offer tight solutions to \emph{data requirement}.
%with the minimum average cost per performance gain by Transfer Learning and fully training of each task to
Meanwhile, to tackle \emph{\challengeIndetrainingcost}, \AlgoNameAbbr\ applies the notion of \emph{dual cost} to estimate real transmission time with bounded error since the optimal time is difficult to obtained. 
%during the task selections. 
Simulation results based on the real visual devices manifest that \AlgoNameAbbr\ outperforms the traditional approaches by 100\%.

%\begin{comment}
\textbf{Paper organization.} 
The rest of this paper is organized as follows. Section \ref{sec: related work} reviews the related works. Sections ? and ? define \ProblemNameAbbr\ and prove the hardness results. We present \AlgoNameAbbr\ and provide the theoretical analysis in Sections ? and ?. Section ? shows the simulation results based on real data. Section VIII concludes this paper.
%\end{comment}
}
%needs to balance the differences resulting from training time, cost and workers available. 
% Fully Training 縮成 FT 好嗎？以及 Transfer Learning 縮成 TL 好嗎？或者有更好的縮法？因為這樣一直出現有點冗
% 定義一下好的optimization problem名稱及其縮寫
% 定義在 Variable.tex 就可以用變數，之後如果修改，也可以無痛一鍵修改
%//可以阿 就前面定義一下 --> 記得取好一點的題目名字XD sexy可能太難了
%// OKOK ，記得改一下喔，我繼續往下看
% 本來想叫你cite昶佑那篇還有另一篇我丟出去的globecom，來讓reviewer覺得我們有做相關的研究，不是亂唬爛的新手，但是仔細想想根本沒意義，因為infocom是double-blind，review期間paper上面不能掛作者名字 //我們submit那個版本不能有名字對吧？y 我剛拿掉了

%以下介紹一下問題：比方說要給定什麼、輸出是什麼、有哪些限制constraint（給constraint名字）
% 下一段講很困難需要權衡的選擇（賣藥，對每個權衡或困難命名），給一個例子解釋為什麼困難，例如：如果都選a，那b那邊會很爛，整體會很爛之類的，且必須要注意每個困難分別對應到那些constraint
% 要小心困難處不能寫成要看很深入才看得懂，要能讓 reviewer 直覺上就看懂
% 接著才講演算法，介紹其效能(ratio），演算法的步驟，每一個步驟都命名，並且指出每個步驟是針對哪一個困難處設計
% 困難的部分你好像已經把一部分整理在下一段，我會去搬上來改
%//這真的不好寫 又要淺又要難
%Multitask Learning is an approach to inductive transfer that improves generalization by using the domain information contained in the training signals of related tasks as an inductive bias. It does this by learning tasks in parallel while using a “shared representation”; what is learned for each task can help other tasks be learned better.

% 要把 reviewer 當笨蛋，要教他們
% 但是這段定義真是有點太難懂...太抽象XD //這段我抄wiki的XD 覺得將得很好 不太好懂是真的
% 我應該有表達到吧？ 但是我覺得太抽象 因為 inductive transfer 變成另一個生字，用生字解釋生字，只會更慘，懂的人看得懂，不懂的人看不懂 orz
% 其實我沒有說你的問題，是說那個定義的問題XD

% 老師我問你一下 我有找到time per image的資料
% //他是只有針對Resnet(encoder)去作實驗，不知道直接把這個當作benchmark行不行
%// 我想說以這個作benchmark來++-- 
%// 他有算1個GPU 跑一張圖要多久 那 假設這是baseline, 來做distribution
% 這樣 ok，你是指 normal distribution 的基礎值//exactly!
% 不過你之前是不是已經找到 ResNet 50
%//他這是tensorflow的網站給的
% 數據你先留著，過幾天專題給我們 result，我們再請他跑另一個 setting
%// 老師 會不會這種時間的預測很不實際 會被reject阿？
% https://researchweb.iiit.ac.in/~jitendra.katta/papers/predicting_training_time_final.pdf
% 這篇快速喵過，再掃一下其他篇，我覺得這個研究一定有
% // 好 我儘快
% 看 abstract 就覺得是我們要的
% 他應該是用一點點 echo 看一開始的 loss function 變化，就可以猜未來多久到達目標threshold
% 所以不用真的把它 train 完，只要跑幾秒就可以估計之類的
% 相較之下，要跑 300 分鐘，幾秒就顯得無所謂，可以看成 training time 可以在短時間內估計
% 也可以明天再繼續弄，今天好像有點晚了
%// 我就算躺下 還是滿腦子這些 晚點睡好 
% XD 我之前也是這樣，滿腦子都是 paper，躺下來以後都是數學符號在飛...
% 找 paper 來 support，確定有方法可以估計
% 「我覺得有 reference 的 setting 都跑跑看，到時候挑那個結果最好的」
% 每張圖都會不一樣嗎？還是平均一張圖
% 是每個 task 都不一樣嗎
% 如果每個 task 都不一樣就可以直接用
% 都一樣的話，那算出的 time 應該也會一樣吧 XD




%6/28 start writing related work, experiment and problems. 




==> Back_ProblemDescription.tex <==
\section{The \ProblemNameAbbr\ Problem} \label{sec: problem description}
%\subsection{Hardness}
This paper considers a mobile edge network that consists of 1) a base station $b$ with a set of antennas $M$ and an edge server which acts as a central server for Federated Learning and 2) a set of smart devices $K$ with \emph{non-identical} computing and transmission capacities for training the shared model from the central server. 

To mitigate the difficulty resulting from different computation time, a hard deadline $\epsilon$ is given. 
{\color{red}
That is to say, if one of selected device cannot send back its update within $\epsilon$, the packet will be dropped. Thus, the release dates of all jobs can be the same at $\epsilon$. Besides, due to $nonidentical$ transmission capacity, each device has its transmission time denoted by $t(i)$, where $i \in K$. However, the total transmission time (denoted by $T$) cannot be summed up directly all the transmission time of each device. Instead, $T$ should be carefully determined by scheduling the devices over $M$ antennas in the BS. Let binary variable $y_{im}$ denote if device $i$ is to be deployed on antenna $m \in M$ and binary variable $x_i$ denote the selection of device $i$ . A device should be assigned to an antenna as long as it is selected.
\begin{align}
    \sum_{m\in M} y_{im} = x_i, && \forall i\in K \label{cons: y = x}
\end{align}
Let $T_m$ denote the transmission time on antenna $m \in M$. It is obviously to see that:
\begin{align}
    T_m = \sum_{i\in K} t(i) \cdot y_{im}, && \forall m\in M \label{cons: T_m}
\end{align}
The transmission time $T$ must be greater than the transmission time of the slowest one among all antennas.
\begin{align}
    T \geq T_m, && \forall m\in M \label{time equation}
\end{align}
For calculating expenditure $C$ for device selection, $C$ is defined as follows: 1) \emph{Computation expenditure} denoted by $c$, represents the expenditure to request a device to train the shared model with its local data. 2) \emph{Data expenditure} denoted by $d_i$, shows the expenditure of the access of the local data of device $i \in K$ for training. The total expenditure can be shown as follows:
\begin{align}
    C =\sum_{i\in K} x_i(c + d_i) \label{expenditure equation}
\end{align}
where $c \in \mathbb{R^+}$ is a constant. It is nature to estimate that mobile devices nowadays have similar computation capabilities.
Consider the amount of data and performance the constraints of data and EMD are listed below:
\begin{align}
    \sum_{i\in K} x_i D_i \geq \mathcal{D} \label{cons: data} 
\end{align}
where $D_i$ and $\mathcal{D}$ represent the amount of data the device $i$ possesses and the given data requirement, respectively. 
Furthermore, \cite{Non-IID} sheds light on the impact of distribution divergence. It is nature to set a threshold $\mathcal{E}$ and 
\begin{align}
    \sum_{i\in K} x_i E_i \leq \mathcal{E} \label{cons: emd} 
\end{align}
where $E_i$ stands for the EMD of device $i \in K$.

\begin{definition}
Given a set of devices $K$,  the data requirement $\mathcal{D}$, data quantity $D_i$ of client $i \in K$ and the computation expenditure $c$, the \ProblemName\ (\ProblemNameAbbr) aims to find a set of devices fully trained for the global model of the server, and schedule the devices to minimize (\ref{time equation})$-$(\ref{expenditure equation}) with the constraints (\ref{cons: y = x})$-$(\ref{cons: T_m}) and (\ref{cons: data})$-$(\ref{cons: emd}) and
\begin{align}
    \min  \mathfrak{R} = \alpha\cdot C + \beta \cdot T \label{obj}
\end{align}
where parameters $\alpha , \beta \in [0,1]$ are tuning knobs (e.g., see the simulation setting in Section \ref{sec: evaluation})
%\footnote{\color{cyan}\textbf{The justification for $\alpha$ needs reference here \cite{??}.}} 
for users to differentiate the importance of completion time and total expenditure.
\end{definition}
After organizing (\ref{obj}), we have the following formulation:

\begin{equation}
\begin{aligned}
& {\text{min}}
& & \mathfrak{R} \\
& \text{subject to}
& & \sum_{i\in K} x_i D_i \geq \mathcal{D}, \\
&&& \sum_{i\in K} x_i E_i \leq \mathcal{E}, \\
&&& x_i\in \{0,1\}.
\end{aligned} \label{OF-MKP}
\end{equation}
}
{\color[RGB]{30,100,30}
\begin{example}  \label{ex:problem}
\begin{table}[t]

\parbox{.48\linewidth}{
\centering 
{\tabcolsep=0.1cm
\caption{Initial value}
\label{tab: Initial value}
\begin{tabular}{|c | c  c  c  c c|} 
\hline
 & $U_1$ & $U_2$ & $U_3$ & $U_4$ & $U_5$\\ [0.1ex] 
\hline
$t(i)$ & 0.6    & 0.5    & 0.4   & 1.9   & 0.2 \\ 
$D_i$  & 450    & 350    & 300   & 550   & 250 \\
$C$    & 0.817  & 0.658  & 0.579 & 0.975 & 0.5 \\
\hline
\end{tabular}
}}
\parbox{.58\linewidth}{
\centering
{\tabcolsep=0.1cm
\caption{Transmission time Group}
\label{tab: Transmission time group}
\begin{tabular}{|c l |c|} 
\hline
\multicolumn{2}{|c|}{Group} & $t(i)$ \\ [0.2ex] 
\hline
$\mathcal{G}_{1}=$ & \{$U_5$\}& 0.2\\ 
$\mathcal{G}_{2}=$ & \{$U_5$,$U_3$\}& 0.4\\
$\mathcal{G}_{3}=$ & \{$U_5$,$U_3$,$U_2$\}& 0.5\\ 
$\mathcal{G}_{4}=$ & \{$U_5$,$U_3$,$U_2$,$U_1$\}& 0.6\\
$\mathcal{G}_{5}=$ & \{$U_5$,$U_3$,$U_2$,$U_1$,$U_4$\}& 1.9 \\
\hline
\end{tabular}
}}
\end{table}
The example shows how to select device, calculate completion time and label expenditure for different solutions, where $K$ includes five devices (i.e, $U_1$, $U_2$, $U_3$, $U_4$ and $U_5$) and two antennas. Table \ref{tab: Initial value} summarizes the initial value.
For example, assume $M=2$, $\alpha=\beta=0.5$, and the given data threshold $\mathcal{D}=800$. At the beginning, we can select the group set by transmission time (see Table \ref{tab: Transmission time group}).
Table \ref{tab: Transmission time group} can acquire sub-group set $\{U_2,U_3,U_5\}$, $\{U_1,U_3,U_5\}$ and $\{U_1,U_3,U_5\}$ for the $\mathcal{G}_{3}$, $\mathcal{G}_{4}$ and $\mathcal{G}_{5}$, by iteratively select device of minimum dual cost $y(\delta)$ until $\sum_{i\in \delta} D_i \geq \mathcal{D}$, and discard this group if $\sum_{i\in \delta} D_i < \mathcal{D}$. 
Then, we can get a sequence of non-increasing by sub-group set (i.e., $\mathcal{G}_{3}$: $\{U_2,U_3,U_5\}$). 
We can schedule by the sequence, such that the device is scheduled the minimum $T$ of the antenna (see Fig. \ref{fig:all_figs_of_example}).
Fig. \ref{fig:all_figs_of_example} compare the solution of our problem \AlgoNameAbbr\ with two traditional approaches, \NaiveFederatedLearning\ and \GreedyClientSelection. \NaiveFederatedLearning\ is random select until $\sum_{i\in K} D_i \geq \mathcal{D}$, and generates the solution to achieve data quantity $550+350=900$ with total cost $0.975+0.658=1.633$ including completion time $1.9$ (in Fig. \ref{fig:NFL_makespan}, antennas 1 and 2 accommodate device 4 and device 2, respectively) and total expenditure $0.5\times(1.633+1.9)=1.7665$.
By contrast, \GreedyClientSelection\ selects device 4 and device 1 by data quantity per cost in decreasing order to achieve data quantity $550+450=1000$ with total cost $0.975+0.817=1.792$ including completion time $1.9$ (in Fig. \ref{fig:GCS_makespan}, antennas 1 and 2 accommodate device 4 and device 1, respectively) and total expenditure $0.5\times(1.792+1.9)=1.846$.
Finally, our algorithm \AlgoNameAbbr\ (detailed later in Section V) selects devices 2, 3 and 5 (i.e., Fig. \ref{fig:TACTIC_makespan}) and only requires the minimum overall cost $0.5+0.658+0.579=1.737$ including completion time $0.6$ (see Fig. \ref{fig:TACTIC_makespan}) and total expenditure $0.5\times(1.737+0.6) = 1.1685$. Compared with \NaiveFederatedLearning\ and \GreedyClientSelection, \AlgoNameAbbr\ reduces total expenditure by $34\%$ and $37\%$ with a speedup of $3.16$x.
Assuming that this model takes 10 times to converge, \NaiveFederatedLearning\ and \GreedyClientSelection\ methods total time spend 19, compared to 6 for \AlgoNameAbbr, and reduce total expenditure by $62.5\%$ and $62.7\%$ with a speedup of $3.16$x. %做10次的時間差距 NFL cost:10.3165; GCS cost:10.396; TACTIC cost:3.8685

\begin{figure}%[t]
        \subfigure[\NaiveFederatedLearning]{\includegraphics[width=.15\textwidth]{graph/NFL.pdf}\label{fig:NFL_makespan}}
        \subfigure[\GreedyClientSelection]{\includegraphics[width=.15\textwidth]{graph/GCS.pdf}\label{fig:GCS_makespan}}
        \subfigure[\AlgoNameAbbr]{\includegraphics[width=.15\textwidth]{graph/TACTIC.pdf}\label{fig:TACTIC_makespan}}
        \caption{Devices scheduling with group sequence}
        \label{fig:all_figs_of_example}
\end{figure}
\end{example}

}

==> NPhard.tex <==
%\section{Hardness Results}
%\label{sec: hardness}

%The classical \ProblemNameAbbr\ is NP-hard .

\ProblemNameAbbr\ is NP-hard since the NP-complete decision version of \emph{Parallel Machine Scheduling Problem} (D-PMS) \cite{DesignApproximation} can be reduced to the decision version of \ProblemNameAbbr\ (D-\ProblemNameAbbr)\footnote{{D-\ProblemNameAbbr} asks whether a solution with a training cost less than a given cost threshold $q$ exists.}
%\footnote{\label{footnote: np-hard}{D-\ProblemNameAbbr} asks whether a solution with a training cost less than a given cost threshold $q$ exists. Obviously, if the optimal solution of \ProblemNameAbbr\ can be obtained in polynomial time, then the solution can be used to answer D-\ProblemNameAbbr. Thus, if D-\ProblemNameAbbr\ is NP-hard, then \ProblemNameAbbr\ is also NP-hard.} 
in polynomial time. The proof is omitted due to the page limit.


\begin{comment}


Theorem \ref{theo: NP-hard} shows that \ProblemNameAbbr\ is NP-hard since the decision version of Parallel Machine Scheduling Problem (D-PMS, which is NP-complete; see Definition \ref{defi: PMSP}), can be reduced to the decision version of \ProblemNameAbbr\ (D-\ProblemNameAbbr)\footnote{\label{footnote: np-hard}{D-\ProblemNameAbbr} asks whether a solution with a training cost not greater than a given cost threshold $q$ exists. Obviously, if the optimal solution of \ProblemNameAbbr\ can be obtained in polynomial time, then the solution can be used to answer D-\ProblemNameAbbr. Thus, if D-\ProblemNameAbbr\ is NP-hard, then \ProblemNameAbbr\ is also NP-hard.} in polynomial time. 
%For ease of reading, we only give the proof sketch as follows.
%The reduction can be done by setting $\alpha=0,\beta=1,D=n$ and transforming $n$ jobs with the processing time $p_1,...,p_n$ and $m$ machines to $n$ devices with the upload time\footnote{\color{red}Although the number of local parameters is fixed for all devices, it is reasonable to set the upload time of each device as above since the transmission rate in the constructed instance can be set to any value.} $t(1)=p_1,...,t(n)=p_n$ and $D(1)=...=D(n)=1$ and $m$ channels, respectively. Then, PMS can be answered by examining whether there is a solution with the training cost not greater than the given threshold $q$. 
%Therefore, \ProblemNameAbbr\ is NP-hard.
%We omit the proof due to page limit.

\begin{definition} \label{defi: PMSP} \cite{DesignApproximation}
%\cite{PMSP}
Given $n$ jobs with processing time $p_1,...,p_n$ and $m$ machines, the \emph{Parallel Machine Scheduling Problem} (PMS) asks for the assignment of $n$ jobs over $m$ machines such that the overall completion time is minimized.
%whether an assignment of $n$ jobs over $m$ machines can finish the $n$ jobs within a given time threshold $q$.
The \emph{decision version} of PMS (D-PMS) asks whether an assignment can finish the jobs within a given time threshold $q$.
\end{definition}

\end{comment}


\begin{comment}
\begin{theorem} \label{theo: NP-hard}
{\ProblemNameAbbr} is NP-hard.
\end{theorem}
\begin{proof}
We show that D-PMS can be reduced to {D-\ProblemNameAbbr} in polynomial time to prove that {\ProblemNameAbbr} is NP-hard.\footnotemark[\ref{footnote: np-hard}]
Given any D-PMS instance with $n$ jobs with processing time $p_1,...,p_n$, $m$ machines, and a given threshold $q$, we construct the corresponding {D-\ProblemNameAbbr} instance as follows.
For each job $i$ with processing time $p_i$ in the D-PMS instance, we create a device $i$ with upload time\footnote{Although the number of local parameters is fixed for all devices, it is reasonable to set the upload time of each device as above since the transmission rate in the constructed instance can be set to any value.} $t(i)=p_i$
%and $D(i)=1$
in the instance of {D-\ProblemNameAbbr}. 
We set both the EMD and the data quantity of each created device to one and create $m$ corresponding channels for the $m$ machines.
By setting $\alpha = 0$, $\beta = 1$, $\mathcal{D}=n$, and $\mathcal{E} = 1$, it is easy to verify that the reduction can be done in polynomial time.
Then, the answer (i.e., yes or no) of the constructed {D-\ProblemNameAbbr} instance with the same threshold $q$ can be used to answer the D-PMS instance and vice versa. Thus, {D-\ProblemNameAbbr} and {\ProblemNameAbbr} are both NP-hard accordingly.
\end{proof}

\end{comment}

==> PseudoCode.tex <==
%\vspace{-0.3cm}

\section{Pseudocode}
\label{appendix: pseudocode}

\begin{breakablealgorithm}
%\begin{algorithm}[h]
    \small
    \caption{\AlgoNameAbbr}
    \label{pseudocode}
    \begin{algorithmic}[1]
    \INPUT
        Data requirement $\mathcal{D}$, 
        skewness threshold $\mathcal{E}$, 
        number of channels $|M|$, 
        set of devices $K$ with 
        data quantity $D(i)$, 
        distribution skewness $E(i)$, 
        upload time $t(i)$, 
        and expenditure $c(i), \forall i \in K$ 
    \OUTPUT
        Selection, scheduling, and training cost of selected devices
    %\State \textbf{Initialize:} SIoT and collaborative group selection $\mathbb{S}=\emptyset$, MEC server selection $\mathbb{M}=\emptyset$, set of collaborative groups $\mathbb{G}=\emptyset$
        \phase{CD Grouping}
        %\ForAll{device $i$ in $K$ with $E(i)\geq \mathcal{E}$}
        %    \State $K \leftarrow K\setminus\{i\}$;
        %\EndFor
        \State Group counter $h\leftarrow 0$;
        \State Sort all distinct upload time of devices in a non-decreasing order;
        \For{each upload time $l$ in the sorted upload time list}
            \State $h\leftarrow h+1$ and $l_h \leftarrow l$;
            %\State Create a group $\mathcal{G}_h=\emptyset$;
            \State Create a group $\mathcal{G}_h=\{i\in K | t(i)\leq l_h \text{ and } E(i)\leq \mathcal{E}\}$;
            %\ForAll{device $i$ in $K$ with $t(i)\leq l$}
            %    \State $\mathcal{G}_h\leftarrow\mathcal{G}_h\cup\{i\}$;
            %\EndFor
            \If{$D(\mathcal{G}_h) < \mathcal{D}$}
                \State Discard $\mathcal{G}_h$;
            \EndIf
        \EndFor
        \phase{CD Gathering}
        \For{each $\mathcal{G}_h$ among all existing groups}
            \State $\delta \leftarrow \emptyset$;
%            \For{each device $i$ in $\mathcal{G}_h$}
            \State $b_i\leftarrow 0$ for each device $i$ in $\mathcal{G}_h$; 
%            \EndFor
            \While{$D(\delta) < \mathcal{D}$ \textbf{and} $\mathcal{G}_h\setminus \delta \neq \emptyset$}
                \State $y_{\delta} = \min_{i\in \mathcal{G}_h\setminus\delta}y_{\delta}(i)$, where $y_{\delta}(i) = \frac{\hat{c}(i)- b_i}{s^\delta(i)}$;
                \State $i^{\delta} = \argmin_{i\in \mathcal{G}_h\setminus\delta} y_{\delta}(i)$;
                \For{each device $i$ in $\mathcal{G}_h\setminus \delta$}
                    \State $b_i\leftarrow b_i + s^\delta(i)\cdot y_\delta$;
                \EndFor
                \State $\delta \leftarrow\delta \cup\{i^\delta\}$;
            \EndWhile
            %\If{$D(\delta) < \mathcal{D}$}
            %    \State Discard $\mathcal{G}_h$;
            %\Else
            \State $\mathcal{G}^t_h \leftarrow \delta$;
            %\EndIf
            
        \EndFor
        \phase{CD Scheduling}
        \For{each $\mathcal{G}_h$ among all existing groups}
            %\State Workload of each antenna $T_m \leftarrow 0$ for all $m\in M$;
            \State $\mathcal{G}^t_h(m)\leftarrow \emptyset$ for each $m\in M$;
            \For{each task $i\in \mathcal{G}^t_h\setminus \bigcup \mathcal{G}^t_h(m)$ with the maximum $t(i)$}
                \State Channel $m^i_h \leftarrow \argmin_{m\in M} \sum_{i\in \mathcal{G}^t_h(m)} t(i)$;
                \State $\mathcal{G}^t_h(m^i_h)\leftarrow\mathcal{G}^t_h(m^i_h)\cup \{i\}$;
            \EndFor
            \State $\tau(\mathcal{G}^t_h) \leftarrow \max_{m\in M} \sum_{i\in \mathcal{G}^t_h(m)} t(i)$;
            \State $c(\mathcal{G}^t_h) \leftarrow \beta \cdot \tau(\mathcal{G}^t_h) + \alpha \sum_{i\in \mathcal{G}^t_h} c(i)$;
        \EndFor
        \phase{FS Selection}
        %\State Selected device set $\mathcal{G}'\leftarrow \emptyset$;
        \State Selected device set $\mathcal{G}' \leftarrow \argmin_{\mathcal{G}^t_h:D(\mathcal{G}^t_h)\geq \mathcal{D}} c(\mathcal{G}^t_h)$;
        \State \textbf{return} Selected device $\mathcal{G}'$ with cost $c(\mathcal{G}')$ and scheduling $\tau(\mathcal{G}')$
    \end{algorithmic}
\end{breakablealgorithm}
%\end{algorithm}


==> RelatedWork.tex <==
\section{Background \& Related Work}
\label{sec: related work}
 

\subsection{Traditional Compressed Sensing Networks} 

In traditional compressed sensing IoT networks, an edge server-assisted architecture is utilized, consisting of multiple edge servers, data aggregators, and a group of IoT devices \cite{amarlingam2018novel,luo2010does}. These IoT devices are organized into clusters based on their location and delay requirements. Each cluster employs a data aggregator, similar to a supervisory control and data acquisition system, to connect the IoT devices to an edge server \cite{zhang2021learning, wang2020collaborative}. When the IoT devices collect raw sensing data, they transmit it to the assigned data aggregator, referred to as intra-cluster transmission \cite{zhang2021learning}. The data aggregator then applies pre-defined measurement matrices to compress the data signals, with the requirement that the measurement matrices must satisfy the restricted isometry property to ensure that the sparsified data signals can be recovered to their original form \cite{candes2008restricted,davenport2010analysis,bandeira2013certifying}. The compression ratio of the measurement matrices also impacts the size of the compressed data. Next, the data aggregator sends the compressed data signals to the edge server through inter-cluster transmission. Upon receipt, the edge server employs greedy iterative-based algorithms \cite{mallat1993matching,tropp2007signal,needell2010cosamp}, convex optimization-based algorithms \cite{chen2001atomic,tibshirani1996regression}, or the augmented Lagrangian alternating direction algorithm \cite{li2013efficient}~ to perform the data reconstruction process. However, these reconstruction algorithms are computationally demanding, and the reconstruction of the compressed data is limited by the dimension and sparsity of the original signals \cite{zhang2021learning}.



\subsection{Deep Compressed Sensing Networks.} 

To address the intensive computation of traditional compressed sensing, deep learning has been integrated into the process. In deep compressed sensing IoT networks, the same edge server-assisted architecture is used but the compression and reconstruction process is replaced by deep learning models \cite{bora2017compressed,wu2019deep,yang2017dagan, ching2020model}. Different models such as denoising autoencoder \cite{vincent2008extracting}, and variational autoencoder \cite{kingma2013auto}~are used for this purpose. Specifically, the data aggregator applies the encoder to encode the raw sensing data from the IoT devices into latent vectors, which have a smaller dimension than the raw sensing data but retain important information. The data aggregator then sends the latent vectors to the edge server for further analysis. The edge server uses the decoder to reconstruct the data from the latent vectors. This process reduces the amount of data transmitted between the data aggregator and edge server and results in better reconstructed data compared to traditional compression methods \cite{zhang2021learning,bora2017compressed}. However, the prevalent deep compressed sensing frameworks mostly adopt an offline learning approach and focus only on the error between original and reconstructed data. Such an offline learning approach restricts access to sufficient training data and hinders adaptivity to diverse reconstruction tasks. The exclusive emphasis on the error may negatively impact the performance of follow-up IoT data-driven DL-based applications.




==> TheoreticalAnalysis.tex <==
\section{Theoretical Analysis} \label{sec: theoretical analysis}

%The time complexity of \AlgoNameAbbr\ ($O(|K|^3)$) is omitted due to page limit. The approximation ratio analysis is as follows.
 
%\begin{comment}
%We analyze the time complexity and the approximation ratio of \AlgoNameAbbr\ as follows.
The time complexity and approximation ratio are as follows.

\begin{complexity} 

\begin{comment}
CD Grouping creates at most $|K|$ different groups. For each group $\mathcal{G}_h$, CD Gathering iteratively selects a device among the $|K|$ devices to obtain a candidate solution $\mathcal{G}_h^t$ with at most $|K|$ devices. For each group $\mathcal{G}_h^t$, CD Scheduling iteratively finds the channel with the lowest workload among $|M|$ ($\leq |K|$) channels\footnote{If $|M|>|K|$, every device can be assigned to a different channel, thereby implying no need for scheduling and further reducing the complexity.} 
%and 
and assigns the device with longest upload time to the found channel.
FS Selection finally selects the best solution among at most $|K|$ candidate solutions.
\end{comment}

The time complexity is $O(|K|^3)$. We omit the details due to page limit. {\AlgoNameAbbr} is efficient and can be accelerated with multiple processors (see Section \ref{sec: evaluation}).
\end{complexity}
%\end{comment}


%\subsubsection{Approximation Ratio.}

\begin{theorem}\label{theo: approximation ratio}
\AlgoNameAbbr\ is a 3-approximation algorithm.
\end{theorem}
\begin{proof}
Let $\mathcal{G}'$ denote the set of devices with training cost $c(\mathcal{G}')$ selected by FS Selection, where all devices in $\mathcal{G}'$ are iteratively selected from group $\mathcal{G}_{h'}$ by CD Gathering (i.e., $\mathcal{G}'=\mathcal{G}^t_{h'}$).
There exist two possible cases for the maximum upload time $l'$ of device set $\mathcal{G}'$. 
Consider the first case, $l'$ is equal to the maximum upload time $l^*$ of device set $\mathcal{G}^*$ selected by the optimal solution, and $l'\neq l^*$ in the second case.
In the following, let $c^*$ denote the optimal training cost.


For the first case, we calculate the upload completion time $\tau(\mathcal{G}')$ for devices in $\mathcal{G}'$.
Since CD Scheduling iteratively assigns the devices with the maximum upload time to the channel with the lowest workload,
the device with the last upload completion time in the scheduling must start transmitting before the time $\frac{\sum_{i\in\mathcal{G}'}t(i)}{|M|}$.
Besides, the upload time length of last device must be no longer than that of the longest one, $\max_{i\in \mathcal{G}'} t(i)$.
Therefore, we know
\begin{align}
c(\mathcal{G}') &= \alpha \sum_{i\in \mathcal{G}'} c(i)+\beta\cdot\tau(\mathcal{G}') \notag\\
& \leq \alpha \sum_{i\in \mathcal{G}'}c(i)+\beta \bigg(\frac{\sum_{i\in\mathcal{G}'}t(i)}{|M|}+\max_{i\in \mathcal{G}'} t(i)\bigg) \notag\\
& = \sum_{i\in \mathcal{G}'} \hat{c}(i)+ \beta \bigg(\max_{i\in \mathcal{G}'} t(i)\bigg) \leq \sum_{i\in \mathcal{G}'} \hat{c}(i)+ c^*. \label{eq: eq1}
\end{align}
The last inequality holds since the optimal solution has a device with upload time $\max_{i\in \mathcal{G}'}t(i)$ in the first case.
Let $y_\delta = 0$ if $y_\delta$ is not set by (\ref{y_delta}) to generate solution $\mathcal{G}'$ and thus we know
\begin{align}
    \sum_{i\in \mathcal{G}'} \hat{c}(i) 
    = \sum_{\delta \subseteq \mathcal{G}_{h'}} y_\delta \sum_{i \in \mathcal{G}' \setminus \delta} s^{\delta}(i). \notag
\end{align}
Let $i_l$ be the last device in $\mathcal{G}'$ selected by \AlgoNameAbbr. 
Thus, $D(\mathcal{G}') \geq \mathcal{D}$ and $D(\mathcal{G}' \setminus \{i_l\}) < \mathcal{D}$. 
Hence, for all the devices $i \in \mathcal{G}' $ except $i_l$, $s^{\delta}(i) = \min\{D(i),\mathcal{D}-D(i)\} = D(i)$ at that time in CD Gathering where $\delta$ was the set of devices at that point. Then, let $R(\delta)=\mathcal{D}-D(\delta)$, and we have
\begin{align*}
    \sum_{i\in \mathcal{G}' \setminus \delta} s^{\delta}(i) 
    = s^{\delta}(i_l) + D(\mathcal{G}'\setminus \{i_l\}) - D(\delta)< 2 R(\delta).
\end{align*}
The last inequality holds since $s^{\delta}(i_l)=\mathcal{D}-D(i)\leq R(\delta)$ and $D(\mathcal{G}' \setminus \{i_l\}) - D(\delta) < \mathcal{D} - D(\delta) = R(\delta)$. Then, we can see that for any $\delta \subseteq \mathcal{G}^*$,
$R(\delta) \leq \sum_{i\in \mathcal{G}^*\setminus\delta} s^{\delta}(i)$.
Thus, due to (\ref{y_delta}),
\begin{align}
    \sum_{i\in \mathcal{G}'} \hat{c}(i) 
    & < 2\sum_{\delta\subseteq\mathcal{G}_{h'}} y_{\delta} R(\delta)
    \leq 2\sum_{\delta\subseteq\mathcal{G}_{h'}} y_{\delta} \sum_{i\in \mathcal{G}^*\setminus \delta} s^{\delta}(i)\notag\\
    &= 2\sum_{i\in \mathcal{G}^*} \sum_{\delta\subseteq \mathcal{G}_{h'}: i\notin \delta} y_{\delta}s^{\delta}(i)
    \leq 2\sum_{i\in \mathcal{G}^*} \hat{c}(i)
    \leq 2c^*. \label{eq: eq2}
\end{align}
By (\ref{eq: eq1}) and (\ref{eq: eq2}), we have $c(\mathcal{G}') \leq 3c^*$. The first case holds.


For the second case, recall that FS Selection examines the candidate solution for each possible maximum upload time length and then selects the one with the minimum training cost.
Since the candidate solution with the maximum upload time length $l^*$ must be examined by FS Selection, $c(\mathcal{G}')$ must be bounded within $3c^*$. The theorem follows.
\end{proof}



\begin{comment}
\noindent\textbf{Extension for the non-identical computing capacity case.}
%To support the generalized case, 
Let $w(i)$ and $q(v)$ denote the training overhead of each task $i\in U$ and the computing capacity of each worker $v\in V$.
% q(v) is normalized to be no less than 1
Thus, the training time of task $i$ on worker $v$ is $t(i,v)=w(i)/q(v)$.
CS Initialization creates the groups $\mathcal{U}_1,...,\mathcal{U}_{m'}$ according to the distinct pairs of $w(i)$ and $q(v)$ to restrict both of the maximum task overhead and the minimum worker computation capacity and $m'$ is at most $|U||V|$.
%for each group $\mathcal{U}_h$.
Let $\mathcal{V}_h\subseteq V$ denote the available workers in $\mathcal{U}_h$, where $h\in[1,m']$.
%instead of $t(i)$ 
CS Gathering then modifies $\hat{c}(i)=\alpha(\frac{w(i)}{\sum_{v\in \mathcal{V}_h}q(v)})+\beta\cdot b(i)$ to generate each $\mathcal{S}_h$.
%Once $|\mathcal{S}_h|\leq |V_h|$, CS Gathering sets $V_h=V_h\setminus\{\tilde{v}\}$ to re-generate $\mathcal{S}_h$ until $|\mathcal{S}_h|\geq |V_h|+1$, where $\tilde{v}=\argmin_{v\in V_h}q(v)$.
For each $\mathcal{S}_h$, CS Scheduling first sorts the source tasks in non-decreasing order of $w(i)$, and then iteratively assigns the source task with the maximum $w(i)$ to the worker in $\mathcal{V}_h$ on which its finishing time will be earliest until no source tasks are left.
Ties are broken by assigning the task to the worker with a higher $q(v)$.
%In this way, the completion time of $\mathcal{S}'$ with its workers $\mathcal{V}'$ in the candidate solution chosen by FS Selection is at most $\frac{\sum_{i\in\mathcal{S}'}w(i)}{\sum_{v\in \mathcal{V}'}q(v)}+\frac{(|\mathcal{V}'|-1)\max_{i\in \mathcal{S}'}w(i)}{\sum_{v\in\mathcal{V}'}q(v)}$.
%$\frac{\sum_{i\in\mathcal{S}'}w(i)+(|\mathcal{V}'|-1)\max_{i\in \mathcal{S}'}w(i)}{\sum_{v\in \mathcal{V}'}q(v)}$.
In this way, 
%Therefore, the approximation 
the approximation ratio of the optimum to the solution selected by FS Selection is
%$\log \gamma+1+\frac{\max_{i\in\mathcal{S}'}w(i)}{\min_{i\in\mathcal{S}^*}w(i)}\cdot \frac{\max_{v\in\mathcal{V}'}q(v)}{\min_{v\in\mathcal{V}^*}q(v)}$.
$\log \gamma+1+ \frac{\max_{v\in\mathcal{V}}q(v)}{\min_{v\in\mathcal{V}^*}q(v)}$.
%Theorem \ref{theo: approximation ratio} also holds for the generalized case. 
The proof is omitted due to the similarity.
%the page limit and similarity.
\end{comment}
